ViMA -- the spinning rotor gauge to measure the viscosity of tritium between 77 and 300 K

Experimental values for the viscosity of the radioactive hydrogen isotope tritium (T$_2$) are currently unavailable in literature. The value of this material property over a wide temperature range is of interest for applications in the field of fusion, neutrino physics, as well as to test ab initio calculations. As a radioactive gas, tritium requires careful experiment design to ensure safe and environmental contamination free measurements. In this contribution, we present a spinning rotor gauge based, tritium compatible design of a gas viscosity measurement apparatus (ViMA) capable of covering the temperature range from 80 K to 300 K.

==> 04_uncertainty_estimation.tex <==
\section{uncertainty estimation}
\label{sec:uncertainties}
\begin{itemize}
    \item T-Stibilisierung aus Referenzmessung ziehen
    \item Teaser für weiteres paper ->Simulationen/Uncertainty-Paper
\end{itemize}
\textcolor{red}{Alexander/Johanna}


==> 06_therm_simu_SRG.tex <==
\section{thermal simulation SRG}
\label{sec:simualtionSRG}

\begin{figure}[t]
    \centering
    \includegraphics[trim = 10mm 0mm 15mm 15mm, width=70mm]{Ansys_H2_5mbar_77K.png}
    \caption{Thermal simulation of the SRG }{The thermal gradient, generated with this simulation of the heat inside the SRG at \SI{77}{\kelvin} and \SI{5}{\milli\bar} is $\approx \SI{2}{\kelvin}$ over a distance of \SI{3}{\milli\meter}. }
    \label{fig:ThermGradientSRG}
\end{figure}

As described in section \ref{sec:measurementprocedure}, during the measurement at one pressure set-point, the rotor is heated up by eddy currents and minor effects. The heat, which is produced for every re-acceleration can be calculated. The formula is derived in \cite{Jousten2018}, where the heat load on the rotor is correlated with the deviation of the normalized deceleration rate, leading to 
\begin{equation}
    Q = c \cdot \rho\cdot V \cdot \frac{\Delta(\nicefrac{\frac{\mathrm{d}\Omega}{\mathrm{d}t}}{\Omega})}{2\alpha}\,,
\end{equation}
where $Q$ is the thermal energy, $c$ is the specific heat capacity, $\rho \cdot V$ the mass and $\alpha$ the thermal expansion coefficient of the SRG rotor. Knowing this, and extracting the values for $\Delta(\nicefrac{\frac{\mathrm{d}\Omega}{\mathrm{d}t}}{\Omega})$ from the measurements, a simple thermal simulation with ANSYS\textsuperscript\textregistered 2020 R2 can be done, to get an upper limit on the temperature gradient inside the sample gas around the rotor. To keep it simple, only the finger, the rotor and the gas inside are simulated. The gasflow inside the finger of the SRG is neglected. To mimic the cooling of the finger, the outer surface of the finger is set to \SI{77}{\kelvin}. The thermal energy is generated as a heat flux through the surface of the rotor, to simulate a perfect heat transfer from the rotor to the gas. The initial temperature of the system is set to \SI{77}{\kelvin}. The load is activated for \SI{1}{\second}, afterwards the system has \SI{12}{\second} to cool down again. This is repeated for \SI{5}{\minute} until the system reaches equilibrium. The gas parameters are adjusted to \SI{77}{\kelvin} and \SI{5}{\milli\bar}. The same is done for helium and hydrogen at \SIlist{77;300}{\kelvin}. The thermal gradient derived from this simulation ranges form \SIrange{0.8}{2.5}{\kelvin}. Knowing, that the measurement results for the viscosity of these gases tends to be slightly higher, than the literature values, the reason might be the heating of the sample gas surrounding the rotor. As mentioned before, this simulation is just giving an upper limit, since the normalised deceleration rate is not only dependent on the heat of the gas, but also on the rotational frequency of the rotor, which has been neglected so far. Additionally the gas inside the finger is not static but moving around the rotor, colliding with the inner wall of the finger. So the thermal heat transfer inside the gas might be faster than for the static case. The impact of this is currently under investigation.

